Error-Aware Imitation Learning from Teleoperation Data for Mobile Manipulation

In mobile manipulation (MM), robots can both navigate within and interact with their environment and are thus able to complete many more tasks than robots only capable of navigation or manipulation. In this work, we explore how to apply imitation learning (IL) to learn continuous visuo-motor policies for MM tasks. Much prior work has shown that IL can train visuo-motor policies for either manipulation or navigation domains, but few works have applied IL to the MM domain. Doing this is challenging for two reasons: on the data side, current interfaces make collecting high-quality human demonstrations difficult, and on the learning side, policies trained on limited data can suffer from covariate shift when deployed. To address these problems, we first propose Mobile Manipulation RoboTurk (MoMaRT), a novel teleoperation framework allowing simultaneous navigation and manipulation of mobile manipulators, and collect a first-of-its-kind large scale dataset in a realistic simulated kitchen setting. We then propose a learned error detection system to address the covariate shift by detecting when an agent is in a potential failure state. We train performant IL policies and error detectors from this data, and achieve over 45% task success rate and 85% error detection success rate across multiple multi-stage tasks when trained on expert data. Codebase, datasets, visualization, and more available at https://sites.google.com/view/il-for-mm/home.

==> fig-tasks_dummy.tex <==
\begin{figure}
\centering
\begin{subfigure}{0.19\textwidth}
\centering
\includegraphics[width=\columnwidth]{example-image-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.19\textwidth}
\centering
\includegraphics[width=\columnwidth]{example-image-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.19\textwidth}
\centering
\includegraphics[width=\columnwidth]{example-image-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.19\textwidth}
\centering
\includegraphics[width=\columnwidth]{example-image-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.19\textwidth}
\centering
\includegraphics[width=\columnwidth]{example-image-a}
\end{subfigure}
\vskip\baselineskip
\begin{subfigure}{0.19\textwidth}
\centering
\includegraphics[width=\columnwidth]{asset/subtask_grab_bowl.png}
\end{subfigure}
\hfill
\begin{subfigure}{0.19\textwidth}
\centering
\includegraphics[width=\columnwidth]{asset/subtask_dump_trash.png}
\end{subfigure}
\hfill
\begin{subfigure}{0.19\textwidth}
\centering
\includegraphics[width=\columnwidth]{asset/subtask_open_dishwasher.png}
\end{subfigure}
\hfill
\begin{subfigure}{0.19\textwidth}
\centering
\includegraphics[width=\columnwidth]{asset/subtask_bowl_in_sink.png}
\end{subfigure}
\hfill
\begin{subfigure}{0.19\textwidth}
\centering
\includegraphics[width=\columnwidth]{asset/subtask_open_drawer.png}
\end{subfigure}
\caption{\textbf{Simulated Kitchen Tasks.} We present 5 challenging long-horizon mobile manipulation tasks. \textit{Top:} Tasks include multi-stage components, requiring varied interactions with multiple household objects. From left to right: Set Table from Dishwasher, Set Table from Dresser, Table Cleanup to Dishwasher, Table Cleanup to Sink, Unload Dishwasher to Dresser. \textit{Bottom:} Diverse manipulation skills are required to solve individual subtasks, such as accurate pick-placements for grabbing the bowl, rotation-heavy motion while dumping trash from the bowl, and operation of constrained mechanisms when opening the dishwasher and searching the drawer. Note that the teleoperator is limited to this ego-centric view, highlighting the partial observability in this setup.}
\label{fig:tasks}
\vspace{-15pt}
\end{figure}
